Angular Stability Analysis of Parallel Connected Grid-following PV Inverters

High penetration of distributed generators (DG) in modern power grids creates angle, voltage, and frequency instabilities. Most of the work in the literature has focused on small-signal stability analysis of single grid-connected inverters without thoroughly investigating their transient stability for large disturbances and interactions between parallel-connected inverters. To address these challenges, this paper examines the transient angular stability of a cluster of grid-following current source inverters. In a low inertia weak grid environment, grid-following inverters may lose synchronism due to faults and large-signal disturbances. A comparison of the voltage injection angle for pre-fault, fault-on trajectory, and post-fault conditions is performed, and an evaluation of the critical fault clearing time is directly related to the uniformity of the aggregated grid-following inverters. The results show that some inverters lose synchronism more quickly than others due to considerable variances in line impedances and apparent power values. Additionally, inverters with high apparent power are more susceptible to losing synchronism due to the maximum current limit, causing the voltage at the point of common coupling to decrease.

==> image.tex <==





\begin{figure}[t]
\centering{\includegraphics[width=1\textwidth,left] {standalone_inverter.pdf}}
\caption{This is an image from a text that uses color to teach music.}
\label{fig}
\end{figure}


\begin{figure}[hbt!]
\centering{\includegraphics[width=.8\textwidth,left] {grid_connected_inverter_final.pdf}}
\caption{This is an image from a text that uses color to teach music.}
\label{fig}
\end{figure}
